Analysis of Flux Corrected Transport Schemes for Evolutionary Convection-Diffusion-Reaction Equations

We report in this paper the analysis for the linear and nonlinear version of the flux corrected transport (FEM-FCT) scheme in combination with the backward Euler time-stepping scheme applied to time-dependent convection-diffusion-reaction problems. We present the stability and error estimates for the linear and nonlinear FEM-FCT scheme. Numerical results confirm the theoretical predictions.

==> solvability.tex <==
\section{Solvability of the FEM-FCT Methods}\label{sec:solvability}
This section provides the existence and uniqueness of the solution for both linear and nonlinear version of the FEM-FCT methods. For the nonlinear scheme, the uniqueness of the 
linearized counterpart, where \(\alpha_{ij}\) are constant independent of \(u\), will be given.
\subsection{Linear FEM-FCT}
The linear version of FEM-FCT can be expressed as 
\begin{equation}\label{eq:system_linear_fem_fct}
M_Lu^n+\tau \mathbb{A}u^n = \tau f^n +M_Lu^{n-1}+f^*(u^{n-1}).
\end{equation}
The matrix \(\mathbb{A}\) is by construction an \(M\)-matrix and \(M_L\) is diagonal matrix with nonzero diagonal entries. This implies that the matrices \(\mathbb{A}\)
and \(M_L\) are invertible. Furthermore, the matrix \(\mathbb{A}\) is strictly diagonally dominant with \(\bar{a}_{ii} >0\) and positiveness of \(M_L\) shows that \((M_L)_{ii}+\bar{a}_{ii}\tau  >0\) and \(M_L + \tau  \mathbb{A}\) is strictly diagonally dominant. This shows that the system matrix is an \(M\)-matrix and hence the problem \eqref{eq:system_linear_fem_fct} has a unique solution. 

\subsection{Non-linear FEM-FCT}
The existence of solution for the nonlinear FEM-FCT scheme follows the same approach as for the steady state convection-diffusion-reaction equations, for more details see~\cite{BJK16}.

\begin{lemma}
Let \(X\) be a finite-dimensional Hilbert space with inner product $(\cdot,\cdot)_X$ and norm $\|\cdot \|_X$. Let $T:X\rightarrow X$ be a continuous mapping, and let $K>0$ be a real number such that $(Tx,x)_X>0$ for any $x\in X$ with $\|x\|_X=K$. Then $\exists\ x\in X$ such that $\|x\|_X<K$ and $Tx=0$.
\end{lemma}
\begin{proof}
For proof see~\cite[Lemma 1.4]{Te77}.
\end{proof}

\begin{theorem}\label{thm:existence_nl}
Let \(A\) be a positive definite matrix. For any \(i,j\in\lbrace 1,\ldots, N\rbrace\), let \(\alpha_{ij}:\mathbb{R}^N\rightarrow [0,1]\) be such that \(\alpha_{ij}(u_1^n,\ldots,u_N^n)(u_j^n-u_i^n)\) and \(\alpha_{ij}(u_1^n,\ldots,u_N^n)[(u_i^n-u_i^{n-1})-(u_j^n-u_j^{n-1})]\) are continuous functions of $u_1^n,\ldots,u_N^n$. Moreover, let \eqref{eq:limiter_symmetry} hold. Then there exists a solution of \eqref{eq:fem_fct} provided the scheme is stable.
\end{theorem}
\begin{proof}
Let \(\underline{u}\equiv (u_1,\ldots, u_N)\) the elements of \(\mathbb{R}^N\). 
Since $A$ is positive definite by assumption, thus one has 
\[
C_A=\underset{\|\underline{u}\|=1}{\mathrm{inf}}\sum_{i,j=1}^Nu_ia_{ij}u_j>0.
\]
Also the mass matrix is positive definite i.e., there exists a constant \(C_M\) such that
\[
\sum_{i,j=1}^Nu_ia_{ij}u_j\geq C_M\|\underline{u}\|^2\quad \forall \underline{u}\in \mathbb{R}^N.
\]
Let us define the operator $T:\mathbb{R}^N\rightarrow \mathbb{R}^N$ by
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n \right)_i&=\sum_{j=1}^Nm_{ij}(u_j^n-u_j^{n-1})+\tau \sum_{j=1}^Na_{ij}u_j^n
+\sum_{i,j=1}^Nm_{ij}(1-\alpha_{ij})\left[(u_i^n-u_i^{n-1})-(u_j^n-u_j^{n-1}) \right]
\\&\qquad+\tau \sum_{j=1}^Nd_{ij}(1-\alpha_{ij})(u_j^n-u_i^n)-f_i^n\tau \ \ \ \ \ \ \ \mathrm{for }\ i=1,\ldots,N.
\end{aligned}
\end{equation*}
Then $\underline{\tilde{u}}^n$ is a solution of nonlinear problem \eqref{eq:fem_fct} if and only if $T\underline{\tilde{u}}^n=0$. 
Using the continuity of $T$ the operator equation has the form
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n,\underline{u}^n\right)&=\tau \sum_{i,j=1}^Nu_i^na_{ij}u_j^n+\sum_{i,j=1}^Nu_i^nm_{ij}(u_j^n-u_j^{n-1}) +\sum_{i,j=1}^Nu_i^nm_{ij}(1-\alpha_{ij})\left[ (u_i^n-u_i^{n-1})-(u_j^n-u_j^{n-1})\right]
\\&
\qquad +\tau \sum_{i,j=1}^Nu_i^nd_{ij}(1-\alpha_{ij})(u_j^n-u_i^n)-\tau (F^n,\underline{u}^n)
\\&=\tau \sum_{i,j=1}^Nu_i^na_{ij}u_j^n
+
\sum_{i,j=1}^Nu_i^nm_{ij}u_j^n-\sum_{i,j=1}^Nu_i^nm_{ij}u_j^{n-1}
 +\sum_{i,j=1}^Nu_i^nm_{ij}(1-\alpha_{ij}) (u_i^n-u_j^n)\\
 &\qquad+\sum_{i,j=1}^Nu_i^nm_{ij}(1-\alpha_{ij})(u_j^{n-1}-u_i^{n-1})
 +\tau \sum_{i,j=1}^Nu_i^nd_{ij}(1-\alpha_{ij})(u_j^n-u_i^n)-\tau (F^n,\underline{u}^n).
\end{aligned}
\end{equation*}
The application of \cite[Lemma 1]{BJK16} for the fourth and fifth term on the right-hand 
side, the positive definite property of matrices, and the Cauchy Schwarz inequality for 
the last term, gives
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n,\underline{u}^n\right)&\geq -\sum_{i,j=1}^Nu_i^nm_{ij}u_j^{n-1}+\sum_{i,j=1}^Nu_i^nm_{ij}(1-\alpha_{ij})(u_j^{n-1}-u_i^{n-1})
 -\tau \|F^n\|\|\underline{u}^n\|+C_A\|\underline{u}^n\|^2+C_M\|\underline{u}^n\|^2
\\&=-\sum_{i,j=1}^Nu_i^nm_{ij}\alpha_{ij}u_j^{n-1}-\sum_{i,j=1}^Nu_i^nm_{ij}(1-\alpha_{ij})u_i^{n-1}
 -\tau \|F^n\|\|\underline{u}^n\|+(C_A+C_M)\|\underline{u}^n\|^2.
\end{aligned}
\end{equation*}
Using $\|Ax\|\leq \|A\|_{\mathrm{Fr}}\|x\|$, where $\|\cdot \|_{\mathrm{Fr}}$ is the Frobenius norm, the above inequality reduces to
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n,\underline{u}^n\right)&\geq -\|M\alpha\|_{\mathrm{Fr}}\|\underline{u}^n\|\|\underline{u}^{n-1}\|-\|M(1-\alpha)\|_{\mathrm{Fr}}\|\underline{u}^n\|\|\underline{u}^{n-1}\|
 -\tau \|F^n\|\|\underline{u}^n\|+(C_A+C_M)\|\underline{u}^n\|^2,
\end{aligned}
\end{equation*}
The stability of the scheme gives $\|\underline{u}^{n-1}\|\leq C_S$ with $C_S$ is the stability constant independent of $\underline{u}^{n-1}$. Using this, we get
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n,\underline{u}^n\right)&\geq -\left(\|M\alpha\|_{\mathrm{Fr}}C_S+\|M(1-\alpha)\|_{\mathrm{Fr}}C_S+\tau \|F^n\|\right)\|\underline{u}^{n}\|
+(C_A+C_M)\|\underline{u}^n\|^2.
\end{aligned}
\end{equation*}
Finally, the Young's inequality for the first term on the right-hand side implies that
\begin{equation*}
\begin{aligned}
\left(T\underline{u}^n,\underline{u}^n\right)&\geq \frac{C_A+C_M}{2}\|\underline{u}^n\|^2-C_0>0,
\end{aligned}
\end{equation*}
where $C_0,C_A,$ and $C_M$ are constants independent of $\underline{u}^n$. Then for any $\underline{\tilde{u}}^n$ satisfying $\|\underline{\tilde{u}}^n\|^2>2C_0/C_A+C_M$ concludes the existence of solution.
\end{proof}

\begin{corollary}
Consider any $\alpha_{ij}\in [0,1]$ satisfying \eqref{eq:limiter_symmetry} independent of the solution $\underline{u}^n$. Then the system \eqref{eq:fem_fct} has an unique solution for any $f_1,\dots,f_N\in \mathbb{R}^N$.
\end{corollary}

\begin{proof}
For constant $\alpha_{ij}$ we get a system of linear equations and hence the solution have to be unique.
\end{proof}

\begin{remark}
For the continuity of $\alpha_{ij}$ in Theorem \ref{thm:existence_nl}, we will us the same result as provided in \cite{BJK16} for the steady state counterpart. For completeness we only mention the result and for the proof we refer to \cite[Lemma 6]{BJK16}.
\end{remark}

\begin{lemma}\label{lemma:alpha_continuity}
Consider any $i,j=1,\dots,N$ and let $\alpha_{ij}:\mathbb{R}^N\rightarrow [0,1]$ satisfy
\begin{equation}\label{eq:alpha_continuity_form}
\alpha_{ij}(\underline{u})=\frac{A_{ij}(\underline{u})}{|u_j-u_i|+B_{ij}(\underline{u})}\ \ \ \ \ \forall\ \underline{u}\equiv (u_1,\dots, u_N)\in \mathbb{R}^b,\ \ u_j\neq u_i
\end{equation}
where $A_{ij},B_{ij}:\mathbb{R}^N\rightarrow [0,\infty)$ are non-negative functions that are continuous at any point $\underline{u}\in \mathbb{R}^N$ with $u_i\neq u_j$. Then $\Phi_{ij}(\underline{u})=\alpha_{ij}(\underline{u})(u_j-u_i)$ is a continuous function of $u_1,\dots,u_N$ of $\mathbb{R}^N$.
\end{lemma}
